Automated Support for Unit Test Generation: A Tutorial Book Chapter

Unit testing is a stage of testing where the smallest segment of code that can be tested in isolation from the rest of the system - often a class - is tested. Unit tests are typically written as executable code, often in a format provided by a unit testing framework such as pytest for Python. Creating unit tests is a time and effort-intensive process with many repetitive, manual elements. To illustrate how AI can support unit testing, this chapter introduces the concept of search-based unit test generation. This technique frames the selection of test input as an optimization problem - we seek a set of test cases that meet some measurable goal of a tester - and unleashes powerful metaheuristic search algorithms to identify the best possible test cases within a restricted timeframe. This chapter introduces two algorithms that can generate pytest-formatted unit tests, tuned towards coverage of source code statements. The chapter concludes by discussing more advanced concepts and gives pointers to further reading for how artificial intelligence can support developers and testers when unit testing software.

==> exercises/q_unit_testing.tex <==
\begin{mdframed}[style=style1]
Exercises: \francisco{I still need to write the answer to these.}
\begin{enumerate}
    \item Write the test cases for invalid weight and age. You can use the \pythoninline{test_invalid_height()} method as a starting point.
    \item Write the test method for the constructor of the BMICalc class. Be mindful to avoid redundancy when checking for invalid valus for constructor arguments.
    \item Would you agree that the code coverage of the \pythoninline{test_bmi_adult()} method is satisfactory? Justify your answer.
    \item Write the methods for testing the remaining age brackets for the children and teens BMI. You can use the \pythoninline{test_bmi_children_4y()} as a reference.
    \item In the \pythoninline{test_bmi_value_valid()}, a colleague suggests to add a second assertion to verify the same BMI classification (e.g., overweight) for a difrerent combination of height, weight and age.
    \begin{itemize}
        \item Do you agree or disagree with that suggestion? Justify your answer
        \item How does the additional assertion impact code coverage? Will the resulting test method increase, decrease or keep the same code coverage?
    \end{itemize}
\end{enumerate}
\end{mdframed}
